Testing geometric representation hypotheses from simulated place cell recordings

Hippocampal place cells can encode spatial locations of an animal in physical or task-relevant spaces. We simulated place cell populations that encoded either Euclidean- or graph-based positions of a rat navigating to goal nodes in a maze with a graph topology, and used manifold learning methods such as UMAP and Autoencoders (AE) to analyze these neural population activities. The structure of the latent spaces learned by the AE reflects their true geometric structure, while PCA fails to do so and UMAP is less robust to noise. Our results support future applications of AE architectures to decipher the geometry of spatial encoding in the brain.

==> tex/0_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Neurons in the hippocampus, entorhinal cortex, and other associated areas were discovered to ‘fire’ (generate action potentials) in response to the spatial location of a moving rat. In particular, pyramidal cells of the hippocampus typically fire when a rat is in a particular location in its environment – they thus indicate or encode information related to the ‘place’ of the animals and were called place cells [2]. The firing patterns of these neurons are recorded by surgically implanting custom multi-electrode recording devices on a rat’s head and moving these electrodes into the brain. When the rat moves in its environment, these electrodes record the electrical activity of nearby neurons and we can later correlate this activity to the location of the rat. Since the discovery of place cells half a century ago, many more cell types (grid cells, border cells, velocity cells, head direction cells) etc. have been discovered to represent information related to other aspects of space and navigation [3]. The activity of these neurons is referred to as the cognitive map [4]. However, recent experiments have found that when a rat undergoes complex behavior, these same neurons encode information not only about space, but also other variables relevant to the animal’s task [5].  (...)
%We do not know the relationship between the structure of the task and the structure of the neural representations of the task. In order toTo quantify this relationship, we need to perform experiments where the animal can be trained on a non-trivial task, its parameters should be changed dynamically, population activity of large numbers of neurons should be recorded, and the structure underlying this neural data should be decoded and correlated to behavioral variables. My thesis project addresses this last challenge. Current neural population decoding techniques rely on linear or nonlinear dimensionality reduction, mathematical techniques that find a low-dimensional approximation of high-dimensional data. While these techniques are powerful and have been used to find evidence of hidden task-relevant states in neural data from rodents, primates and humans, they tend to discover local properties and not global structure of the cognitive map. A method that can discover parameterizations of the global structure would allow us to compare it to the experimentally determined task structure.
%\myworries{text from MItacs application, to be updated. Introduction not more than 1 page}
\myworries{cut intro by half (half a page). Aim of paper + tools}
\msmcom{Agreed with Khanh}


==> tex/1_methods.tex <==
\section{Methods}
\label{sec:methods}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{2D maze configurations for recording place field cells associated with rodent moving trajectories}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We simulate the activity of place field cells from a rat moving inside 2D mazes, whose design is directly inspired from our lab experiments \textcolor{red}{ref?}. More precisely, the mazes are composed of a subset of connected octagonal tiles, built over the same platform that contain 7$\times$7 tiles in total (see Figure \ref{fig:maze}a). For a given maze with $n$ tiles $\left\{ T_1, \ldots, T_n \right\}$, we model the motion of a rat by setting up a goal (reward) position $g \in \mathbb{R}^2$, and generate random trajectories by simulating a discrete random walk that is biased towards the $g$. as follows: Assuming that the rat is located at position $x \in \mathbb{R}^2$ in tile $i$, we simulate the next move by first computing the shortest sequence of tiles leading to $g$ starting from tile $i$, and selecting the next tile in this sequence. Then, we %For a given maze, we generate random trajectories by simulating a random walk, where at each time fixed step, the next move is obtained by both uniformly sampling the direction over $\left\{0, \ldots, 359 ^\circ \right\}$, and sampling the amplitude according to a \textcolor{red}{XXX distribution (gaussian?)}. 
To simulate the neural activity of $N$ place field cells, we also sampled $N$ points over the maze using a \textcolor{red}{XXX distribution (which one?)}  %associated with the movement of the rat inside a given maze,

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Firing rate function}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For a given place field located at $c$, and a given position $x$ of the rat, we simulate the firing rate $FR(x,c)$ with additive Gaussian white noise as 

\begin{equation}
    FR(p,c) =  FR_{max} \exp\left[-\frac{1}{2} \sqrt{\frac{d(x,c)}{\sigma}}\right] + \varepsilon \mathcal{N}(0,1),
    \label{eq:firing_rate}
\end{equation}
where $d$ is a distance function over the maze, $FR_{max},\sigma >0$ and $\varepsilon>0$ and $\mathcal{N}(0,1)>0$ is a standard Gaussian white noise. In practice, we used $FR_{max}=, \ \sigma= $ and $\varepsilon= $. The firing rate function depends on the choice of the distance used to represent the relative position of the rat with respect to the neuron. We consider here the two following geometric hypothesis:   %and $f$ is a  Gaussian function centered in $0$:
    %$f(d) = \nu_{max} \exp{(-\frac{1}{2} \sqrt{\frac{d}{\sigma}})} + noise$.
    
    \begin{enumerate}
        \item \emph{Euclidean hypothesis}: The distance between is the 2D Euclidean distance $d= \| \cdot \|_2 $. %place cells encode the 2D euclidean position of the rat on the platform.
        \item  \emph{Graph hypothesis}: $d=d_{graph}$ TO compute the distance, we choose (...) This distance is invariant over (...)  
    \end{enumerate}
    
    
  
    
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
\subsection{Auto-Encoder}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
T0 analyze the data, we trained an auto-encoder (AE) that takes a neural state as input (i.e. the firing rate of $N$ neurons, rescaled to (...)),  with 


The firing rates are first rescaled between 0 and 1 through min-max feature scaling. \newline
The encoder and decoder are fully connected networks (4 hidden layers of sizes 64, 32, 16 and 8). The encoder's output layer is $M$-dimensional, where $M$ is the desired dimension of the latent space \myworries{specify $2$ ?}. All hidden layer have leaky ReLU as activation function. The encoder's output layer has a linear function and the decoder's activation function is a Sigmoid. \newline
Two AE are trained separately on the Euclidean data set and on the graph data set. The datasets are split into training validation and testing sets (70\%, 20\% and 10\% respectively). Training is performed in batches of 32 data points, using the ADAM optimizer. The learning rate is initialized to 1e-3 and reduced by a factor 10 on plateaus. 


 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\subsection{Implementation and Code Availability}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The code was developed using Python 3.8.0. The Auto-Encoder design and training was performed using PyTorch 1.11.0 and PyTorch-Lightning 1.6.5. All the codes and datasets are available at \url{https://github.com/NC4Lab/maze_analysis} (\myworries{make repo public}.). %To recover the datasets and trained models or to generate custom data, please refer to file \textsc{readme}.md  \newline


% \subsection{Synthetic data}
% To investigate the nature and structure of cognitive maps in rodents, a platform made of 7x7 octagonal tiles was designed. The platforms allows to create different maze configurations (\myworries{add ref?}). \newline 
% All maze configurations have the geometry of a graph: a home tile is connected to a central node; the central node  leads to $3$ goal tiles. This graph structure is translated and rotated in the platform space, the angle between edges and the length of the edges vary across maze configurations. (\myworries{refer to figure}).\newline
% We generate synthetic data in the different maze configurations. The synthetic data contains trajectories of a virtual rat moving within the maze environments and firing rates of $N$ place cells during those trajectories. Place cells typically fire in a specific region of the behavior space, known as a place field. Place fields generally have a center where the firing rate is the highest; the firing rate decreases progressively as the distance to the center increases. Here, the different maze configurations are used to generate synthetic place cell data under two hypothesis. \newline 
% Under the \textbf{Euclidean hypothesis}, place cells encode the 2D euclidean position of the rat on the platform. The firing field centers have fixed 2D coordinates across all maze configurations.
% Under the \textbf{graph hypothesis}, place cells encode the graph geometry of the maze, in spite of any rotation, translation or distortion of the maze geometry. The maze is separated into $4$ edges. Each place cells is associated to an edge, as well as to a relative position along this edge. A place field center is always located along the same edge, at the same relative distance between the two nodes of this particular edge. Eventually a random lateral shift is added to each place field center. This way, if the graph geometry of the maze is rotated, translated or distorted, the place fields positions vary accordingly. \myworries{add ref to figure} 

% \paragraph{Trajectories generation}
% Two different types of trajectories can be generated: random walks and point-to-point trajectories. During random walks, the step's length randomly varies around a baseline value and the direction of the next step is randomly chosen among $360$ discrete angles ranging from 0 to 359 degrees. \newline
% Point-to-Point trajectories are generated as biased random walks. A starting tile (home) and an end tile (goal) are required as inputs. Knowing the maze configuration, a Breadth-First-Search algorithm is applied to find the shortest path between the home tile and the goal tile. Steps in the direction of goal tile have a higher probability to be taken. 

% \paragraph{Place cells} 
% The firing rate of a particular place cell $i$ at time step $n$ is defined as follows:
% \begin{equation*}
%     \nu_i(n) = f(d(p_n, c_i)) 
% \end{equation*}
% where $p_n$ is the position of the rat at step $n$, $c_i$ is the position of the place field center of the $i$th neuron, $d$ is a distance function and $f$ is a function that maps the distance to a firing rate. $f$ is a  Gaussian function centered in $0$:
%     $f(d) = \nu_{max} \exp{(-\frac{1}{2} \sqrt{\frac{d}{\sigma}})} + noise$. \newline
% The distance function used under the Euclidean hypothesis is the euclidean norm. Under the graph hypothesis, the distance function is the euclidean norm as well, however if the graph distance is beyond a threshold, the firing rate is set to $0$.
% (\myworries{need to specify piece-wise function?}),  (\myworries{add ref to figure, try to have an example of a neuron that is close in2d space but far in graph space}.
% \paragraph{Data set} For each goal and each maze configuration, $15$ point-to-point trajectories (home to goal) are generated. The firing rates of $N = 150$ neurons are generated for each visited position. This is performed separately for the two hypothesis, which results in two sets (Euclidean dataset and Graph dataset) of dimension \textit{$P$x$N$}, where $P$ is the number of positions visited by the virtual rat. 

% \subsection{Auto-Encoder}
% As a means to analyse the dimensionality and structure of the generated data, an Auto-Encoder (AE) is designed.  The AE takes a neural state as input, i.e. a $N$-dimensional vector containing firing rates of $N$ neurons at a specific position. The firing rates are first rescaled between 0 and 1 through min-max feature scaling. \newline
% The encoder and decoder are fully connected networks (4 hidden layers of sizes 64, 32, 16 and 8). The encoder's output layer is $M$-dimensional, where $M$ is the desired dimension of the latent space \myworries{specify $2$ ?}. All hidden layer have leaky ReLU as activation function. The encoder's output layer has a linear function and the decoder's activation function is a Sigmoid. \newline
% Two AE are trained separately on the Euclidean data set and on the graph data set. The datasets are split into training validation and testing sets (70\%, 20\% and 10\% respectively). Training is performed in batches of 32 data points, using the ADAM optimizer. The learning rate is initialized to 1e-3 and reduced by a factor 10 on plateaus. 



% \subsection{Implementation and Code Availability}
% The code and data sets are available at \url{https://github.com/NC4Lab/maze_analysis} (\myworries{make repo public}.). To recover the datasets and trained models or to generate custom data, please refer to file \textsc{readme}.md  \newline
% The code was developed using Python 3.8.0. The Auto-Encoder design and training was performed using PyTorch 1.11.0 and PyTorch-Lightning 1.6.5.





==> tex/2_results.tex <==
\section{Results}
% \myworries{one figure for maze + traj + firing fields. one fig corresponding firing rates. }
% \myworries{One fig for results interpretation; PCA, stat, AE}
% \myworries{should data generation and analysis be separated in 2 different figures? -> yes}


\subsection{Simulating recordings of place field cells according to different representations}


 a home tile is connected to a central node; the central node  leads to $3$ goal tiles. This graph structure is translated and rotated in the platform space, the angle between edges and the length of the edges vary across maze configurations.
XXXXXX

We generated two datasets that (...) 1/ three mazes 
Specify, mazes, number of trajectories, number of neurons hypothesis tested.  


\begin{figure}[h!]
    \centering
    \includegraphics[width=1\textwidth]{figures/fig1_abstract_v2.jpg}
    \caption{Example of generated trajectories \myworries{perhaps add firing field centers and example of firing rates vs time for a specific neuron}}
    \label{fig:maze}
\end{figure}


\subsection{Title}

XXXXXXXXXXXXXXXXXX

\begin{figure}[h!]
   % \includegraphics{figures/double_column_example.png}
    \caption{Difference between Euclidean and Graph hypothesis}
    \label{fig:my_label}
\end{figure}

